Theme-driven Keyphrase Extraction to Analyze Social Media Discourse

Social media platforms are vital resources for sharing self-reported health experiences, offering rich data on various health topics. Despite advancements in Natural Language Processing (NLP) enabling large-scale social media data analysis, a gap remains in applying keyphrase extraction to health-related content. Keyphrase extraction is used to identify salient concepts in social media discourse without being constrained by predefined entity classes. This paper introduces a theme-driven keyphrase extraction framework tailored for social media, a pioneering approach designed to capture clinically relevant keyphrases from user-generated health texts. Themes are defined as broad categories determined by the objectives of the extraction task. We formulate this novel task of theme-driven keyphrase extraction and demonstrate its potential for efficiently mining social media text for the use case of treatment for opioid use disorder. This paper leverages qualitative and quantitative analysis to demonstrate the feasibility of extracting actionable insights from social media data and efficiently extracting keyphrases using minimally supervised NLP models. Our contributions include the development of a novel data collection and curation framework for theme-driven keyphrase extraction and the creation of MOUD-Keyphrase, the first dataset of its kind comprising human-annotated keyphrases from a Reddit community. We also identify the scope of minimally supervised NLP models to extract keyphrases from social media data efficiently. Lastly, we found that a large language model (ChatGPT) outperforms unsupervised keyphrase extraction models, and we evaluate its efficacy in this task.

==> notes/general_notes.tex <==
[notes from Sarah]
============5/7/2023==================
discussion:
--model cost analysis (computational, financial)
--where is the expert in the loop?: before keyword extraction, after keyword extraction (for validating candidate keywords)

============Older notes==================
misinformation pointer:
--pregnancy and sub: https://www.reddit.com/r/suboxone/comments/mrqfmp/suboxone_and_pregnancy/ (this post is in our dataset)

--quick tapering and its underlying cause: loss of job and insurance
--splitting dosage
--reluctance with high dosage

==============================
do we need to mention if, when and how the dataset will be shared?
==============================
--generalizability of or approach: mention in broader impact: not overclaim in the intro

--disentangle the methods and results for RQs.
--the title should highlight that we are doing theme-driven keyword extraction (question-contingent keywords). Also mention the following:
--salient topics of conversation/ help seeking
--way of indexing?
--the same word can be keyword in one post and not a keyword in another post 
-Goal of this work: propose a mixed-method framework to allow researchers to define context-specific keywords: that will allow them to reduce the signal-to-noise ratio

-highlight that we are developing a qualitative coding process to develop a training dataset to apply to help to develop ML / NLP solution

-Future work: 
    currently, we have categories from researchers. In the future, come up with seeds from the researchers:
    -identify network of concepts

--keyword can be very rare in the doc but very important in the meaning of the text
--keyword type annotation needs  modification and review

--should cite health-related new task/dataset papers where the annotators are social media users (not physicians): e.g., Opioid treatment discovery paper @CHI, COVID-HeRa


===================================

Some key points to be considered.
\begin{itemize}
    \item Why is opiate recovery important?
    \item Why can the social media (Reddit) important?
    \item Which aspects (data, methods etc.) are currently missing in this area?
    \item How are we addressing the issues?
    \item What is our core contribution here?
\end{itemize}

\section{Background and Related Works}
To be added.

\section{Problem Formulation}
We are initially interested in the following research questions.
\begin{itemize}
    \item RQ1: How does the set of keywords vary among the posts for different help-seeking online (Reddit) posts?
    
    \item RQ2: How does the set of keywords vary between the posts and the corresponding comments for different help-seeking online (Reddit) posts?
    
    \item RQ3: How does the set of keywords vary for the posts and comments along with the time?

\end{itemize}
Here are some idea
\begin{itemize}
    \item Uncovering the treatment options using 
    \item Characterizing 
    \item Which keywords of the posts promote strong peer engagement?
\end{itemize}

==> notes/omar_notes.tex <==

\section{Notes on content engagement}

\paragraph{RQ1:} What are the most popular discussion keyphrases observed on opioid recovery forums? Which keyphrases provoke the most user engagement and why? Is there synergy between popular keyphrases and content-engagement? 

\paragraph{Part1:} \textcolor{blue}{What are the most popular keyphrases observed in the opioid recovery forums?}

Figure \ref{fig1} shows the 20 popular (frequent) words in the dataset. All the the keyword are normalized and figure \ref{fig2} shows wordcloud representation of all the keyphrases. 

\begin{figure}[h!]
\centering
\includegraphics[scale=0.5]{Note-images/popular-keyphrases.png}
\caption{20 most popular keyphrases}
\label{fig1}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[scale=0.4]{Note-images/normalized_keywords.png}
\caption{Wordcloud representation of normalized keyphrases}
\label{fig2}
\end{figure}

\textbf{Q1:} \textcolor{blue}{Does the presence of keywords increase the engagement in a post?}

Here, engagement in a post is measured in terms of number of comments and upvotes it received. The relation between keyphrases and (comments/upvotes) is presented in Figure \ref{fig3}. From the figures we can see that there exists somewhat positive correlation. 
%As the number of keyphrases increases and engagement also increases. 

\begin{figure}[h!]
\centering
\includegraphics[scale=0.38]{Note-images/cmnt_vs_keywords.png}
\includegraphics[scale=0.38]{Note-images/cmnt_vs_upvotes.png}
\caption{Relation between \#of comments, \#of upvotes and \#of keyphrases [(Left: scatter plot), (Right: mean of scatter values)]}
\label{fig3}
\end{figure}




\textbf{Q2:} \textcolor{blue}{Do post lengths biases the presence of keywords?}

[checking whether long posts tend to have more keywords than shorter posts]. Figure \ref{fig5} shows a positive correlation between length of post and presence of keypharses in a post. Longer posts is likely to have more keywords in it, and such posts usually has more comments and upvotes in it.

\begin{figure*}[h!]
\centering
\includegraphics[scale=0.45]{Note-images/length_cmt_upvotes.png}
\caption{Relation between \#of upvotes and \#of keyphrases}
\label{fig5}
\end{figure*}

\paragraph{Q3:} \textcolor{blue}{How can we measure the user-engagement of keyphrases?}

\textcolor{red}{I think how do we measure the use-engagement of keyphrases will be one of the important point to present in the paper clearly: need some discussion}.

For now, the engagement score of keypharses is calculated in terms of average number of comments, upvotes and (comment+upvotes)[\textcolor{red}{Professor you mentioned about applying some form on normalization when adding comments and upvotes values. Can you kindly give a hint how can I do that?}] a post received in the presence of that keypharses. Engagement score calculation process is described in \ref{Algorithm1}. Figure \ref{fig6} shows the engagment score of top@10 popular words.

\begin{algorithm}[h!]
\SetAlgoLined
\caption{Engagement score calculation process}
\label{Algorithm1}

\textbf{Input:} Set of Keyphrases and Post\\
\textbf{Output:} Engagement score for each Keyphrase\\
\BlankLine
$T \gets \{k_1, k_2, ..., k_m\}$ (set of keyphrases)\;
$P \gets \{p_1, p_2, ..., p_m\}$ (set of posts)\;
$E_c=[]$ (Engagement score based on \#of comments)\;
$E_u=[]$ (Engagement score based on \#of upvotes)\;
$E_{cu}=[]$ (Engagement score based on \#of comments and upvotes)\;

\BlankLine
\For{$k_i \epsilon K$}{
$t_c=0,\;t_u=0\;t_{cu}=0, occur=0\;$ \; 
\For{$p_i \epsilon P$}{
    $ls\gets[]$ (keyphrases of $p_i$)\;
    \BlankLine
\If{$(k_i \; is \;in \; ls)$}{
        $t_c+=n_c$ (adding \#of comments of $p_i$)\;
        $t_u+=n_u$ (adding \#of upvotes of $p_i$)\;
        $t_{cu}+=n_c+n_u$ \;
        $occur+=1$ (updating is occurances)\;
        }
    }
    //updating engagement score.\;
    $E_c.append(t_c/occur)$\;
    $E_c.append(t_u/occur)$\;
    $E_c.append(t_cu/occur)$\;
}
\end{algorithm}


\begin{figure*}[h!]
\centering
\includegraphics[scale=0.5]{Note-images/engagement_socre.png}
\caption{Engagement score of top 10 popular keyphrases (please check the code for getting values for top@50)}
\label{fig6}
\end{figure*}

\paragraph{Q4:} \textcolor{blue}{Does their exists any direct correlation between popularity of keyphrases and their engagement score?}

To find out whether their exists any direct correlation I plotted the top@50 popular keyphrases form the dataset in terms of both \#of comments and \#of upvotes. Figure \ref{fig7} shows the values. From the plot it is evident that engagement does not directly correlate with the popular keyphrases.

Figure suggests that if a keyphrases is popular (frequent) it does not guarantee that post will be more engaging. Less popular keyphrases can have high engagement score.

\begin{figure*}[h!]
\centering
\includegraphics[scale=0.4]{Note-images/com_upvote_eng_bar.png}
\includegraphics[scale=0.4]{Note-images/com_upvote_eng_line.png}
\caption{Engagement score of top 30 popular keyphrases in terms of \#comments, \#upvotes, and \#upvotes+\#comments \textcolor{red}{[same graph is plotted twice just for getting better interpretation]}}
\label{fig7}
\end{figure*}

\paragraph{Part2:} \textcolor{blue}{Which keyphrases provoke the most user engagement and why? Is there synergy between popular keyphrases and content-engagement?}

Figure \ref{fig8} shows the top@40 engaging keywords \#comments, \#upvotes, \#comments+upvotes. \textcolor{red}{Why these keyphrases are have high engagement score? Need discussion }


\begin{figure*}[h!]
\centering
\includegraphics[scale=0.4]{Note-images/eng_score_comment.png}
\includegraphics[scale=0.4]{Note-images/eng_score_upvotes.png}
\includegraphics[scale=0.4]{Note-images/eng_score_comments+upvotes.png}
\caption{Top@50 engaging keywords in terms of \#comments, \#upvotes, \#comments+upvotes}
\label{fig8}
\end{figure*}

\paragraph{Q5:} \textcolor{blue}{Is occurrences of keyphrases biasing the engagement score?}

To check this I have plotted the occurrences of most engaging keyphrases. From figure \ref{fig9} it is clear that, number of occurrences have an impact on engagement score. Top 30 most engaging keywords mostly occured 1-2 times in the dataset. We can see that highest engagement score is 138 and these keyphrases appeared only once in the whole dataset.

\begin{figure*}[h!]
\centering
\includegraphics[scale=0.4]{Note-images/occurance.png}
\includegraphics[scale=0.7]{Note-images/occurance_vs_engagement-score.png}
\caption{ Occurrences of Top@300 engaging keywords in the dataset}
\label{fig9}
\end{figure*}

\paragraph{Q6:} \textcolor{blue}{Which type of keyphrases are more engaging?}

Initially we defined several criteria of Keyphrases. By analyzing the keyphrases we can try to understand which type of keyphrase provoke more engagement.

Such as finding out whether treatment options (dr, endocrinologist, volumetric dosing, kratom,) keyphrases are more engaging then substance use history (benzo, H, pain meds, ...) keyphrases

We can do it after labelling our keyphrases. I have just plotted the values for some keyphrases to get an idea how it will look.
\begin{figure}[h!]
\centering
\includegraphics[scale=0.7]{Note-images/engagement_type.png}
\caption{Which type of keyphrases are more engaging?}
\end{figure}

==> sections/4_Normalization.tex <==
\subsection{Normalization}
Reddit users commonly use various unique phrasings of the same word, e.g., shorthand, slang, and misspellings. For example, the opiate \textit{heroin} may also be referred to as \textit{h}, \textit{dope}, \textit{smack}, and \textit{speedball}, and also it is often misspelled as \textit{herion}, \textit{heroine} etc. For this study to draw general conclusions about MOUD forum discussions, we must identify the meaningful and relevant keyphrases, map the misspelled keyphrases to the correct ones, and normalize all keyphrases to a common parent term. We manually map all keyphrase variations to their most meaningful representative parent phrases to solve this problem. In our analysis, we thus ensure that different slang terms for drugs like \textit{suboxone} (\textit{sub}, \textit{zub}, \textit{bupe}) or \textit{oxycodone} (\textit{contin}, \textit{oxy}, \textit{perc}) are mapped to a common term. Additionally, we normalize terms from all non-treatment categories with examples such as \textit{muscle pain} (\textit{tore a muscle}, \textit{muscle aches}, \textit{muscle tension}), \textit{sobriety} (\textit{sober}), \textit{heart rate} (\textit{high heart rate}, \textit{low heart rate}), and \textit{memory issues} (\textit{memory problems}, \textit{memory loss}, \textit{short term memory problems}). The steps and guidelines we followed to normalize keyphrases are
described in the appendix.%illustrated in this section.  

% \noindent

% \section{Categorization}

% That's why we mapped the normalized keyphrases into the four categories detailed in the Keyphrase Definitions (\textcolor{magenta}{Depends on whether this section exists}) section above. 

% \begin{itemize}joint
%      \item treatment options: Keyphrases that are related to treatments such as treatment name (e.g., medication-assisted treatment), treatment provider (e.g., doctor), way of treatment (e.g., volumetric dosing), elements of treatment (e.g., drug names), etc. were categorized as 'treatment options'.
%     \item 
%     substance dependency and recovery: 
%     Keyphrases related to the long-term usage of a substance belongs to this category. The purpose of the substance usage can be broad, including addiction (e.g., addiction to Heroin), withdrawal management (e.g., suboxone for managing opioid withdrawals), pain mitigation (e.g., oxycodone for pain management), and relaxation (e.g., coffee). If a drug is prescribed by the doctor as part of the treatment or being used by the user for short-term as part of the self-treatment, then it would be a part of the treatment options.
%     \item medical history: This category includes keyphrases concerning the diagnosis of a disease (e.g.,  COVID, hepatitis C) or any particular condition (e.g., pregnancy, appendix removed)  as well as any pre-existing history (e.g., asthma, ADHD, allergy). This category covers medical history beyond substance dependency/recovery
%     \item side effects/psychophysical effect: Any psychological (e.g., depression, anxiety) or physical (e.g., back pain, restless legs and arms) side effects due to the use of substance or medicine falls into this category. WE also identify terms indicating potentially severe side effects as keyphrases, e.g., 'life-threatening'.
%     % \item others: All the keyphrases (e.g, colostrum, scum) that do not show any evidence to fall in the above four categories belong to this category.
% \end{itemize}
%For each normalized keyphrase group (the representative keyphrase along with other keyphrases mapped to it)
%For each normalized keyphrase group (the representative keyphrase along with other keyphrases mapped to it), we considered all the posts that include at least one of the keyphrases of the group. Based on the usage contexts of these keyphrases in the posts, we categorized that keyphrase group. For example, if the keyphrases of a group appeared as 'substance dependency and recovery' in five posts and as 'treatment options' in two posts, we classified that keyphrase group as 'substance dependency and recovery.' In order to check the validity of the categorization, a subset of the generated keyphrase categories was verified by the experts.
% \textbf{Categorization} 

% % substance use, treatment options, medical history, and psychophysical effects are the primary focuses of our keyphrase categorizations. By categorizing keyphrases, we can provide a more low-level analysis of MOUD discussion trends, leading to clearer clinical insights. 
% For each normalized keyphrase, we assign it to one of our categories after a manual review of the keyphrase's context in a sample of posts. 

% If a keyphrase is assigned to multiple categories in different posts, then we assign the more frequent category as the category for that keyphrase. For example, if a keyphrase was assigned to \textit{substance dependency and recovery} in five posts and \textit{treatment options} in two posts, we assigned it as \textit{substance dependency and recovery}. For the rare cases where there was a tie between two categories, the annotation team consulted to find the The final list of categorized keyphrases was shown to and verified by an expert.

% \iffalse It is not uncommon to get different contexts and such indicating different categories for a single keyphrase group. In those cases, we considered the most number of appearing category.\fi
% From the annotation, we obtained a total of 881 unique keyphrases after normalization. The distribution of the keyphrases among different groups can be found in Table \ref{table:keyphrase-cat-ex}. We observed that the highest frequency keyphrase category is “psychophysical effect” with 331 in total. The high prevalence of “psychophysical effect” could be because users were discussing different types of effects they had faced due to the concurrent treatment or substance use, thus seeking suggestions. In contrast, we found the lowest number (35) of keyphrases in the “medical history” category. The possible reason is that users focused on the ongoing problems or effects rather than considering any medical history. It is interesting to get a good amount (182) of treatment options, which indicates that users were concerned about their treatments and thus tried different treatment options. We also found reasonable evidence (77) of keyphrases related to “substance dependency and recovery”. The 255 keyphrases we did not find to be relevant were categorized as “others”.

% \textcolor{magenta}{Alternative passage, only including the examples from each category} 

\noindent



==> sections/X_Research_Questions_old_.tex <==
\section{Research Questions}



\begin{enumerate}
    \item Filter (Maybe) / Definitely normalize the keyphrases after extraction.  
    \item mTurk annotation of keyword-classes 
    \item Plot distribution of topics after normalization.
    \item Plot topic vs engagement. We can define peer engagement as one or more (or all) of the following: (i) number of comments, (ii) number of upvotes, (iii) number of unique users in the comment thread, (iv) number of interactions (comments, replies) from the original poster/ help seeker.
    \item Maybe plot only the uncommon terms? 
    \item Maybe some kind of specific qualitative analysis of a certain keyword that provokes some interesting finding 
\end{enumerate}
\paragraph{Visualizations:}
\begin{enumerate}
    \item Visualizing the list of keywords (top 15) [Post Normalization]
    \item Column for each category of keywords
    \item Topic vs Popularity/Engagement 
\end{enumerate}
\paragraph{Evaluation: } 
\begin{enumerate}
    \item Label the ground truth dataset with classes 
    \item report RQ1 results on ground truth + silver labeled classes from model prediction. 
\end{enumerate}


\subsection{RQ2: What insights can we uncover from analysis of keyphrase co-occurances?}

% \textcolor{purple}{[Ideas from Joey]
% \begin{enumerate}
%     \item Introduce why we care about co-occurrence. What does it signify? 
%     \item A section on general interesting findings. What occured together the most and why is it important? 
% \end{enumerate}
% }
\subsubsection{Aligning Keyphrase Co-Occurrence with Clinical Findings}
We find that self-reports from r/suboxone often discuss the  treatment/side-effect relationships discussed in clinical suboxone guidelines. In fact, there is at least one instance of the keyphrase \textit{suboxone} co-occurring with each of the known adult side-effects listed on the U.S. Substance Abuse and Mental Health Service Administration webpage \footnote{https://www.samhsa.gov/medication-assisted-treatment/medications-counseling-related-conditions/buprenorphine}. This relationship to established substance abuse guidelines validates the quality of our data and annotation guidelines. Additionally, the presence of such annotations allows one to gather a large number of self-reports based on suboxone and a corresponding psycho-physical effect. This facilitates analysis on the context and severity of various suboxone side effects. For example, one user posted: 

\begin{displayquote}
My last dose was Friday and i'm just wondering how much longer im going to feel like dying if i don't take subs again. \textbf{chest pain} sucks,feels like \textbf{heartburn x100 that nothing will take away}, \textbf{stomach pain} is 9/10, \textbf{cold sweats} and \textbf{chills}, everything aches and just \textbf{no energy} to even sit up.
\end{displayquote}

\noindent This post provides feedback on the severity and co-occurrence of common suboxone side-effects.  Automatic identification of posts containing popular medication side-effects can help researchers aggregate low-level information on drug response at scale. This can motivate future research on treatment options and side effect management. 


We additionally note that there are numerous side-effects which are \textit{not} officially listed as known psycho-physical responses to suboxone. For example, almost 2\% of user posts in \MODELNAME expressed issues with their sex drive. For example: 

\begin{displayquote}
I have been on suboxone on and off for about ten years. I am 28 now and have absolutely \textbf{no sex drive} to speak of.  Any ideas other than stopping suboxone. Also I have a problem with sweating profusely. Other than a little insomnia these are the only downsides I have experienced  personally. Any help would be greatly appreciated.
\end{displayquote}

Another side-effect not found on standard suboxone guidelines is \textit{hair loss}. Consider the following post: 

\begin{displayquote}
    ...I do have bleached hair, it's damaged. I do lose a bit to shedding every time I shower/ brush it. However. Today I lost a significant amount, far more than usual. I very well could be trying to chalk it up to coming off subs when it could be a mix of damaged hair, poor diet (too much caffeine and not enough home cooked meals lately) plus this, the timing is just weird.
\end{displayquote}

While this user does seem to provide a non-suboxone explanation for hair loss, the comment section validates the user's experience: 

\begin{displayquote}
    My hair started to feel bleached and fried while I was on subs and started to fall out more than normal. It did continue while I quit at first but started to go back to normal. (3 Upvotes)
\end{displayquote}

Such posts/discussions on medical self-reports can uncover new adverse drug reactions that drive future research in the space of opioid recovery treatment. Thus, the \MODELNAME dataset promotes development of KE tools that allow for future analysis of new psychophysical effects at scale. 

% \subsection{RQ2 }
% \begin{enumerate}
%     \item Topics that appear before/after covid 
%     \item Analysis of why we think that happens ( maybe with supporting citations from clinical opioid literature?) 
% \end{enumerate}
% \paragraph{Visualizations}
% \begin{enumerate}
%     \item Plot keywords over time 
%     \item table:  keyword | representative post with keyword 
% \end{enumerate}

\subsubsection{[RQ3] Keyphrases before and after the onset of the pandemic}
\textcolor{gray}{Basic points: 
\begin{enumerate}
    \item Explain how pre vs. post-pandemic insight is an example analytical lens. This choice is one of many example avenues of exploration. 
    \item Clinical evidence (what does this mean)
    \item Lack of access to medical resources during the pandemic (especially in-person meetings and support/groups). 
    \begin{enumerate}
        \item Treatment option availability and type (drug, behavioral).
    \end{enumerate}
    \item Drug use changes/patterns
    \item Transportation difficulty
    \item COVID risk fears
    \item Pull examples from the dataset to ground the qualitative claims. 
    \item Look for side effect changes related to before/after the pandemic.
\end{enumerate}}
    
A variety of analytical lenses can be applied to \MODELNAME and future datasets created via our methodology. For example, one such dimension of \MODELNAME available to us is the temporal component of our data. Opioid use and abuse are subject to and influenced by global changes [evidence?]. One such global event that had a large impact on opioid use was the COVID-19 pandemic [2 or 3 evidences required]. 

We can divide the \MODELNAME dataset along the date of the COVID-19 pandemic---the 11th of March, 2020---as declared by the WHO \cite{domenico_vanelli_2020}. Comparisons can then be made between the frequencies of keyphrases before and after, shown in figures\textcolor{red}{xx}.


\subsection{RQ4: Peer Engagement \textcolor{orange}{[Omar]}}

In recent years, Reddit has become a place for sharing recovery experiences of different drug usage and providing support to peers \cite{OpioidRecovery,forum77}. The success of any peer discussion group heavily depends on the engagement between the members \cite{Sharma_Choudhury_Althoff_Sharma_2020}. Unfortunately, very few researches have been conducted from the natural language processing perspective on how users interact or seek support in opioid recovery discourse on Reddit. This work aims to compensate for the deficiency by characterization of a user's experience with opioid abuse and recovery by analyzing the keyphrases of user posts on opioid recovery subreddits. In this subsection, we briefly describe the frequent discussion keyphrases in opioid recovery forums, which keyphrases provoke more user engagement and the synergy between frequent keyphrases and engagement. 
 
 \textcolor{blue}{What are the most frequent keyphrases observed in the opioid recovery forums?}
 From the annotation, we obtained two different sets of keyphrases: union and intersection. The union set comprises of all the keyphrases marked by both annotators while the intersection set only contains those keyphrases that exactly match for both annotators. Our empirical observation of frequent keyphrases reveals that people mostly discuss different treatment options (suboxone, sublocade), the psycho-physical effect treatments (anxiety, sleep), and previous substance usage history (oxycodone, heroin) in the opioid recovery subreddit. Table \label{frequent_keyphrase} shows the ten most frequent discussion keyphrases in the dataset.  
\begin{table}[h!]
\begin{center}
\small
%\begin{tabular}{L{1.3cm}C{1cm}C{1cm}C{1cm}C{1cm}}
\begin{tabular}{C{2.1cm}C{1.5cm}|C{2.1cm}C{1.5cm}}
\hline
\multicolumn{2}{c}{\textbf{Union}} & \multicolumn{2}{c}{\textbf{Intersection}}\\
\hline
 \textbf{Keyphrase}  & \textbf{Frequency} & \textbf{Keyphrase} & \textbf{Frequency} \\
 \hline 
suboxone & 690 & suboxone & 609\\
withdrawal & 257 & withdrawal & 149\\
taper & 190 & taper & 92\\
doctor & 117 & subutex & 75\\
buprenorphine & 97 & buprenorphine & 74 \\
opiate & 88 & heroin & 62\\
heroin & 85 & oxycodone & 54\\
oxycodone & 82 & kratom & 51\\
subutex & 79 & fentanyl & 42\\
sleep & 68 & opiate & 41\\
kratom & 66& methadone & 37\\
 \hline
\end{tabular}
\caption{Ten most frequent keyphrases in the dataset. Frequency is measured based on the number of times a keyphrase appeared in the dataset. Multiple occurrences in a post are counted once.}
\label{frequent_keyphrase}. 
\end{center}
\end{table}

\textcolor{blue}{Which keyphrases provoke the most user engagement and why?} Reddit facilitates discussion in a thread-like setting where a user starts the conversation by posting and others interact via comments, upvotes, and downvotes. We modeled the engagement of a post by comments and upvotes parameters. To quantify the amount of attention a keyphrase receives we calculate the engagement score following the algorithm
\ref{Algorithm1}. 


\begin{algorithm}[h!]
\SetAlgoLined
\caption{Engagement score calculation process}
\label{Algorithm1}

\textbf{Input:} Set of Keyphrases and Post\\
\textbf{Output:} Engagement score for each Keyphrase\\
\BlankLine
$T \gets \{k_1, k_2, ..., k_m\}$ (set of keyphrases)\;
$P \gets \{p_1, p_2, ..., p_m\}$ (set of posts)\;
$E_c=[]$ (Engagement score based on \#of comments)\;
$E_u=[]$ (Engagement score based on \#of upvotes)\;
%$E_{cu}=[]$ (Engagement score based on \#of comments and upvotes)\;

\BlankLine
\For{$k_i \epsilon K$}{
$t_c=0,\;t_u=0\;, occur=0\;$ \; 
\For{$p_i \epsilon P$}{
    $ls\gets[]$ (keyphrases of $p_i$)\;
    \BlankLine
\If{$(k_i \; is \;in \; ls)$}{
        $t_c+=n_c$ (adding \#of comments of $p_i$)\;
        $t_u+=n_u$ (adding \#of upvotes of $p_i$)\;
        %$t_{cu}+=n_c+n_u$ \;
        $occur+=1$ (updating is occurances)\;
        }
    }
    //updating engagement score.\;
    $E_c.append(t_c/occur)$\;
    $E_c.append(t_u/occur)$\;
    %$E_c.append(t_cu/occur)$\;
}
\end{algorithm}



\begin{figure*}[b!]
  \centering
  \subfigure[\#Comments]{\includegraphics[scale=0.48, height=9.5cm, width=6.5cm]{figures/engaging_comment_union.png}}\quad
  \subfigure[\#Upvotes]{\includegraphics[scale=0.48, height=9.5cm, width=6.5cm]{figures/engaging_upvote_union.png}}\quad

\caption{Top@30 engaging keyphrases in terms of \#comments, \#upvotes in the union of keyphrases list}
 \label{figunion}
\end{figure*}

\begin{figure*}[b!]
  \centering
  \subfigure[\#Comments]{\includegraphics[scale=0.48, height=9.5cm, width=6.5cm]{figures/eng_comment_inter.png}}\quad
  \subfigure[\#Upvotes]{\includegraphics[scale=0.48, height=9.5cm, width=6.5cm]{figures/eng_upvote_inter.png}}\quad

\caption{Top@30 engaging keyphrases in terms of \#comments, \#upvotes in the intersection of keyphrases list}
 \label{figinter}
\end{figure*}


Figure \ref{figunion} and \ref{figinter} show the top@30 engaging keyphrases in terms of the number of comments and upvotes for union and intersection keyphrase lists respectively. 

%\textcolor{blue}{Does the presence of keyphrases in a post provoke more engagement?} \textcolor{red}{is this a valid question to argue?} actually, I am trying to make a claim that if a post has more keyphrases, it is more likely to attract more users to the discussion. \textcolor{red}{[can discuss in group meeting if seems appropriate]}

\paragraph{}
\textcolor{blue}{Is there synergy between frequent keyphrases and content-engagement?}  To find out whether there exists any direct correlation, we plotted the top@30 popular keyphrases from the dataset in terms of both the number of comments and  upvotes in figure \ref{fig7}. From the plot, it is evident that engagement does not directly correlate with the frequency of the keyphrases. Figures suggest that if a keyphrase is frequent, it does not guarantee that the post will be more engaging. Less popular keyphrases can have high engagement scores.

\textcolor{blue}{What are the implications of these results?}

\begin{figure*}[b!]
\centering
\includegraphics[scale=0.6]{figures/frequent_union.png}

\includegraphics[scale=0.6]{figures/frequent_inter.png}

\caption{Engagement score of top 30 frequent keyphrases in terms of  \#comments and \#upvotes.}
\label{fig7}
\end{figure*}



%\paragraph{An idea:} \textcolor{blue}{Which type of keyphrases are more engaging?} [\textcolor{red}{need discussion}]

%Initially we defined several criteria of Keyphrases. By analyzing the keyphrases we can try to understand which type of keyphrase provoke more engagement. Such as finding out whether treatment options (dr, endocrinologist, volumetric dosing, kratom,) keyphrases are more engaging then substance use history (benzo, H, pain meds, ...) keyphrases

%We can do it after labelling our keyphrases. I have just plotted the values for some keyphrases to get an idea how it will look.


\subsection{RQ5: How Effective Are Off-The-Shelf Keyphrase Extraction Models on \MODELNAME?}

In this section, we investigate the performance of 10 keyphrase extraction methods on the \MODELNAME dataset. This section is organized as follows: First we introduce our baseline methods. Next, we describe our experimental setup. Finally, we provide a discussion of our experimental results.  
\subsection{Baseline Models }
\subsubsection{Statistical Methods} We evaluate the performance of two statistical methods, TfIdf \cite{tfidf} and YAKE \cite{yake}. In TfIdf, keyphrases are ranked based on their frequency in a post. In YAKE, each candidate keyphrase is ranked based on various statistical features including term frequency, position in document, and letter casing. 
\subsubsection{Graph-Based Methods} We explore four different graph-based approaches to keyphrase extraction, namely TextRank \cite{textrank}, TopicRank \cite{TopicRank}, PositionRank \cite{positionrank}, and MultipartiteRank \cite{DBLP:journals/corr/abs-1803-08721}. These models operate on graphical representations of the text, where each candidate keyphrase is a node with edges determined by some syntatic or semantic structure (e.g. a dependency tree). These models are commonly used as baselines in UKE literature \cite{DBLP:journals/corr/abs-2109-07293}, \cite{DBLP:journals/corr/abs-2110-06651}. 

\subsubsection{Embedding Methods} All of our embedding methods use the following three-step pipeline: 1) Extract candidate keyphrases, 2) Embed each candidate and the full reddit post 3) Return the top-k candidate keyphrases with the highest cosine similarity to the embedding of the full reddit post. We evaluate the performance of DistilBERT \cite{distilbert}, BERT \cite{BERT}, DeBERTa-v3 \cite{deberta}, and SBERT \cite{sbert}, as they are all widely-used transformer models with proven ability to produce meaningful contextual word embeddings.
\\
\subsubsection{Experimental Setup}
All models evaluated in this study are unsupervised, as the dataset is too small for supervised learning. For the statistical and graph-based methods, we use the PKE library \cite{pke} to perform keyphrase extraction. For the embedding methods, we use KeyBERT \cite{grootendorst2020keybert} to extract and rank keyphrases. All models use the same candidate keyphrases. Specifically, we use PKE's grammar selection tool to extract only noun-phrases as candidates for each post\footnote{We use the following grammar: \{\<ADJ\>*\<NOUN \mid \mathrm{PROPN \>+}\}}. We report the Recall @ k for each model. All metrics are computed using Scikit-Learn \cite{scikit-learn}. 


\subsubsection{Results} 
Our experimental results find that the SBERT-embeddings produce the highest recall across all experiments. This is expected as 1) Embedding approaches are unique in producing contextual representations of the full post, which explicitly encode textual semantics--- a useful feature in UKE 2) SBERT is the only embedding method employed which was trained to output embeddings for longer sequences of texts (other methods are only explicitly trained to produce only high quality token embeddings). Graph based methods all performed consistently lower than SBERT at all values of k. The method which achieved the 2nd best performance, TfIdf, displays the viability of a low computational cost  method for use in resource constrained settings. 

Unfortunately, none of the standard unsupervised KE models were able to achieve recall above 0.56. This limits the use of off-the-shelf models to draw insights from silver-labeled samples across all of r/suboxone. Large-scale data collection using our described annotation guidelines can enable the use of supervised training which may alleviate this problem. Additionally, social media-specific UKE models may better handle long self reports filled with informal user-generated language. Improving the performance of UKE models on \MODELNAME will be the focus of future works. 



\begin{table}[!h]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{1}{c}{Model}   & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c}{R@15} \\ \midrule
\textbf{Statistical Methods}&                           &                              &      \\ \midrule
TfIdf                       &  0.38                     & 0.50                         & 0.55                         \\ 
YAKE                        &  0.35                     & 0.48                         & 0.51                         \\
\\
\textbf{Graph-Based Methods}&                           &                              &                              \\ \midrule
TextRank                    &  0.16                     & 0.33                         & 0.43                         \\
TopicRank                   &  0.30                     & 0.44                         & 0.49                         \\
PositionRank                &  0.28                     & 0.42                         & 0.50                         \\
MultipartiteRank            &  0.32                     & 0.46                         & 0.52                         \\ 
\\
\textbf{Embedding Methods}  &                           &                              &                             \\ \midrule
DistilBERT                  &  0.30                     & 0.45                         & 0.52                         \\ 
BERT                        &  0.31                     & 0.46                         & 0.52                         \\ 
DeBERTa-v3                  &  0.26                     & 0.39                         & 0.47                         \\ 
SBERT                       &  0.40                     & 0.51                         & 0.56                         \\ 
\bottomrule
\end{tabular}
\caption{Recall @ K for each model. Note: On average only [X]\% of annotated keyphrases appear in the candidate keyphrases, thus max recall is very low. }
\end{table} 



==> weaknesses_and_improvements.tex <==
\section{Weaknesses and Improvements}
List out the main weaknesses and areas that could be improved in this paper (while it's still fresh in our minds). We can begin to address these before our reviewer feedback and certainly afterwards.

\begin{enumerate}
    \item Need more data.
    \item Need a more solid and complete analysis of the extracted keyphrases.
        \item Quantitative analysis and strong differentiation of our keyphrases. 
    \item Didn't try to run a large or more SOTA model (because of the lack of data).
    \item Didn't prove that this would help researchers in the real world, just showed how it's plausible qualitatively. 
    \item Only one subreddit?
    \item Table 1 presents the frequency of keyphrases for different thematic categories. However, the authors have not stated whether it is for the union/intersection keyphrase list.

    \item For addressing questions in RQ1, which keyphrase list have authors utilized: union, intersection or both? How the results differ by using union and intersection keyphrase list

    \item Need some justification for whether sample selection is biasing the results. Most of the keyphrases are from the psychophysical effects and treatment options category that's why results are also more correlated to these two types of keyphrases. How might the qualitative analysis differ if there were more samples for other classes?  (Again related to dataset size)

    \item Can we think a bit more in the peer-engagement direction? (How many of the comments satisfy the information need of the actual post? Can we utilize our TIN classification idea here? Which type of treatment information is a user asking for? How many people comment to give that information?)

    \item Co-occurrence of two keywords have been discussed. We may search for potential co-occurences of multiple keyphrases. Do they show any interesting characteristics? Also, searching for negative correlation (e.g., Is increase of a keyphrase associated with the decrease of another keyphrase?)
    \item Finding out more interesting categories.
    \item Temporal analysis part can be improvement (e.g., presenting a stronger rationale behind the decrease of certain keyphrases, finding out relations between the keyphrase that have increased or decreased after covid-19, etc.)
\end{enumerate} 
